A Formal Framework For Probabilistic Unclean Databases

Most theoretical frameworks that focus on data errors and inconsistencies follow logic-based reasoning. Yet, practical data cleaning tools need to incorporate statistical reasoning to be effective in real-world data cleaning tasks. Motivated by these empirical successes, we propose a formal framework for unclean databases, where two types of statistical knowledge are incorporated: The first represents a belief of how intended (clean) data is generated, and the second represents a belief of how noise is introduced in the actual observed database instance. To capture this noisy channel model, we introduce the concept of a Probabilistic Unclean Database (PUD), a triple that consists of a probabilistic database that we call the intention, a probabilistic data transformator that we call the realization and captures how noise is introduced, and a dirty observed database instance that we call the observation. We define three computational problems in the PUD framework: cleaning (infer the most probable clean instance given a PUD), probabilistic query answering (compute the probability of an answer tuple over the unclean observed instance), and learning (estimate the most likely intention and realization models of a PUD given a collection of training data). We illustrate the PUD framework on concrete representations of the intention and realization, show that they generalize traditional concepts of repairs such as cardinality and value repairs, draw connection to consistent query answering, and prove tractability results. We further show that parameters can be learned in practical instantiations, and in fact, prove that under certain conditions we can learn a PUD directly from a single dirty database instance without any need for clean examples.

==> sections/inference.tex <==
\newcommand{\ol}[1]{\overline{#1}}

\subsection{Cleaning}
\alaslkkl
Our first result relates cleaning in tuple-insertion PUDs to the
traditional notion of minimum subset repairs.  We consider a
tuple-insertion PUD $(\scs,\M,\D,J^\star)$ where $\M=(\K,\Phi,w)$.  We
denote by $\delta_{\D}$ and $\delta_{\K}$ the value generators of $\D$
and $\K$, respectively, and by $q_{\D}$ and $q_{\K}$ the
tuple-selection probability of $\D$ and $\K$, respectively.  For
$i\in\tids(R^J)$ we use the following notation.
\begin{align*}
p_{\D}(i)\eqdef&q_{\D}\cdot\prod_{A\in\sig(R)}\delta^{R.A}_{\D}(R^{J^\star}[i].A)\\
p_{\K}(i)\eqdef&q_{\K}\prod_{A\in\sig(R)}\delta^{R.A}_{\K}(R^{J^\star}[i].A)\\
\ol{p_{\K}}(i)\eqdef &1-p_{\K}(i)
\end{align*}

We now prove the following theorem.
\begin{theorem}
  Let $(\scs,\M,\D,J^\star)$ be a tuple-insertion PUD with
  $\M=(\K,\Phi,w)$, and suppose that for all $i\in\tids(R^J)$ it is
  the case that $p_{\K}(i)>p_{\D}(i)\cdot\ol{p_{\K}}(i)$.  There
  exists a number $M$ such that if $w(\varphi)>M$ for $\varphi\in\Phi$
  then the following are equivalent for all subsets $I$ of $J^\star$.
  \begin{enumerate}
    \item $I$ is a most likely repair.
    \item $I$ is a minimum repair w.r.t.~$\Phi$ for the weighted
      database $\left(J^\star,\log(\frac{p_{\K}}{p_{\D}\ol{p_{\K}}})\right)$.
  \end{enumerate}
\end{theorem}
\begin{proof}
  Let $(\scs,\I,\R,J^\star)$ be the PUD represented by
  $(\scs,\M,\D,J^\star)$.  With the notation we introduced in this
  section, we have the following.
  \begin{align*}
  \prob_{\R\circ\I}(I,J^\star)=& \left(
%
\prod_{i\in\tids(I)}p_{\K}(i)
%
\times
%
\frac{1}{Z}
%
\prod_{\varphi\in\Phi}\prod_{\rho\in\tau(\varphi,I)}
%
e^{-w(\varphi)}
%
\right)\\
&
%
\times
%
\left(
%
\prod_{i\in\tids(J^\star)\setminus\tids(I)}
\ol{p_{\K}}(i)\cdot p_{\D}(i)
\right)
\times
(1-p_{\D})^{|\tids(\D)\setminus\tids(J^\star)|}
% 
\end{align*}

Clearly, if $w$ is large enough, even a single $e^{-w(\varphi)}$
reduces the probability below every database $I$ in which $\Phi$ is
fully satisfied. Now, suppose that $\Pi$ is indeed fully
satisfied. Since we fix $J^\star$ and compare between the $I$s, we can
eliminate the factors that do not depend on $I$. Hence, we get the
following.

  \begin{align}
\notag  \prob_{\R\circ\I}(I,J^\star) \,\,\sim \,\, &
%
\prod_{i\in\tids(I)}p_{\K}(i)
%
\times
%
\prod_{i\in\tids(J^\star)\setminus\tids(I)}
\ol{p_{\K}}(i)\cdot p_{\D}(i)\\
\notag & =
\left(\prod_{i\in\tids(J^\star)}\ol{p_{\K}}(i)\cdot p_{\D}(i)\right)
\times
\left(
\prod_{i\in\tids(I)}\frac{p_{\K}(i)}{\ol{p_{\K}}(i)\cdot p_{\D}(i)}
\right)
\\ \label{eq:max-subset}
\,\,\sim \,\, &  
\prod_{i\in\tids(I)}\frac{p_{\K}(i)}{\ol{p_{\K}}(i)\cdot p_{\D}(i)}
% 
\end{align}
Hence, $I$ is a most likely repair if and only if $I$ satisfies $\Phi$
and maximizes~\eqref{eq:max-subset}, which is the same as maximizing
the sum $\sum_{i\in\tids(I)}\log(\frac{p_{\K}(i)}{\ol{p_{\K}}(i)\cdot
  p_{\D}(i)})$, as claimed.
\end{proof}



==> sections/intro-pud.tex <==
We introduce a formal framework for probabilisitic data cleaning. Our
framework is based upon the concept of a \e{Probabilistic Unclean
Database} (\e{PUD}). Intuitively, a PUD consists of a dirty database
$J\str$, along with a two-step generative model that describes how
dirty databases are distributed; the first step samples a clean
database, and the second introduces noise. We refer to the
distribution that produces the intended clean database as the
\e{intention model} (or just \e{intention} for short), and the
distribution that introduces noise for realising the actual observed
database is the \e{realization model} (or just \e{realization} for
short). The PUD represents a probability distribution over the
possible clean databases---this is the posterior probability given the
observation $J\str$.

More formally, a PUD is a triple $(\I,\R,J\str)$, where $\I$, the
intention, is a probabilistic database, and $\R$, the realization,
maps every sample $I$ of $\I$ to a probabilistic database $\R_I$
(obtained from $I$ by introducing noise), and $J\str$, the
observation, is a dirty database. The models $\I$ and $\R$ define
probability space $\R_{\I}$ over pairs $(I,J)$, and the PUD
$(\I,\R,J\str)$ defines a probabilistic database over $I$s by
conditioning $\R_{\I}$ on $J=J\str$. 

To make the case for the PUD framework, we define three computational
tasks that are driven by real-life motivation. The first problem is
\e{cleaning}, which we capture as a \e{maximum-likelihood inference}:
given $(\I,\R,J\str)$, compute a database $I$ that maximizes the
probability $\R_{\I}(I,J\str)$; we call such $I$ a \e{Most Likely
  Intention} (MLI). The second problem is \e{probabilistic
  query answering}, namely, evaluate a query $Q$ on the probabilistic
cleaning result induced by $(\I,\R,J\str)$. Here, we adopt the
traditional semantics of query answering over probabilistic databases
as \e{marginal inference} where the goal is to determine the marginal
probability of each possible query
answer~\cite{DBLP:conf/vldb/DalviS04,Suciu:2011:PD:2031527}. The third
problem is \e{PUD learning}: given a collection $T$ of examples
$(I,J)$, find the parameters of $\I$ and $\R$ that maximize the
\e{log-likelihood} (sum-of-logs/product of the probabilities) of $T$.
For learning to be well defined, we assume that $\I$ and $\R$ have
\e{parametric} representations $\I_{\Xi}$ and $\R_{\Theta}$, where
$\Xi$ and $\Theta$ are vectors of symbolic parameters, such that
actual $\I$ and $\R$ are obtained by assigning numeric values to the
parameters.

The definition of a PUD is abstract, as it includes only the semantics
of $\I$ and $\R$, and does not mention how they are represented.
Statistical models are typically represented compactly, classic
examples being graphical models and exponential (factor-graph) models
that restrict the correlation between random variables. We illustrate
our framework by instantiating it with two specific representation
systems for PUDs. In both representations, the intention model is a
probabilistic database that we call a \e{Markov
  Logic Database} (MLD), which we explain next. The two
representations differ in their realization. In an \e{MLD/subset} PUD,
the realizer can introduce new tuples; hence, the clean database is
assumed to be a subset of $J\str$. In an \e{MLD/update} PUD, the
realizer can update table cells; hence, the clean database is assumed
to be obtained from $J\str$ by changing cell values.

In an MLD, each tuple is generated independently via a probabilistic
\e{tuple generator}, and in addition, we have weak (and hard)
constraints. The constraints affect the probability of a database in
the sense of Markov random fields~\cite{DBLP:books/daglib/0066829},
namely, each \e{grounding} of the rule adds a multiplicative factor to
the probability. In an MLD, the constraints are \e{Denial Constraints}
(DCs)~\cite{DBLP:journals/jiis/GaasterlandGM92}, phrased in tuple
relational calculus, and each grounding is obtained by assigning
tuples to the free variables. These constraints include the Functional
Dependencies (FDs) and \e{conditional}
FDs~\cite{DBLP:conf/icde/BohannonFGJK07} that are traditionally used
in data repairing~\cite{DBLP:series/synthesis/2011Bertossi}.

We establish several preliminary results on MLD/sub\-set PUDs and
MLD/update PUDs. In particular, we show configurations of the two
where MLIs coincide with \e{minimum
  repairs}---\e{cardinality repairs}~\cite{DBLP:conf/icdt/LopatenkoB07}
in the case of MLD/subset, and \e{optimal
  V-repairs}~\cite{DBLP:conf/icdt/KolahiL09} in the case of
MLD/update. Consequently, for these configurations we immediately
establish complexity results on PUDs from past literature on the
complexity of computing a minimum
repair~\cite{DBLP:conf/icdt/LopatenkoB07,DBLP:conf/icdt/KolahiL09,DBLP:conf/icdt/AfratiK09,DBLP:journals/corr/abs-1708-09140}.
In addition, we show that over MLD/subset PUDs, an MLI can be computed
in polynomial time in a well studied
scenario~\cite{DBLP:journals/tods/KoutrisW17,DBLP:conf/icde/AndritsosFM06,DBLP:journals/ipl/KolaitisP12},
namely there is a single key constraint. Interestingly, unlike
traditional (non-probabilistic) repairs, here the key constraint may
be \e{weak} (e.g., two people are unlikely, but might, have the same
first and last name), and the required MLI may, in fact, violate it.

We also give a result that relates probabilistic query answering on
MLD/subset PUDs to the traditional \e{consistent} query
answering~\cite{DBLP:series/synthesis/2011Bertossi,DBLP:conf/pods/ArenasBC99}
on cardinality repairs. A fundamental difference between the two is
that in the latter, only the cardinality repairs determine
the result (i.e., the set of consistent answers), while in
the former, \e{every subset} of tuples is a possible world that can
take a portion of the probability of an answer. We show that, under
symmetry assumptions, the consistent answers for cardinality repairs
coincide with the answers that approach (at the limit) \%100 certainty
as \e{(a)} the weight of the constraints approaches infinity, \e{and
  (b)} the error probability (i.e., the probability that the realizer
introduces new tuples) approaches zero.

For learning, we focus on MLD/update PUDs and establish the following. In the presence of labeled
examples, learning the parameters of a PUD translates to a
convex optimization problem; consequently, this problem can be solved
in polynomial time \e{if} probabilistic inference (computation of
marginal probabilities) is tractable.  For example, we show that when tuples are
are independent, learning is
solvable in polynomial time via standard optimization methods such as
Stochastic Gradient Descent (SGD). In fact, we show that SGD is (with
high probability) guaranteed to recover the true parameters of a tuple-independent 
PUD within error $\epsilon$ with access to
$O(\epsilon^{-2})$ labeled examples.

\eat{ For learning, we establish the following results. We show that
in the presence of labeled examples, learning for any MLD/update
PUD---this corresponds to PUDs with arbitrary
constraints---corresponds to a convex optimization problem and that
PUD learning can be solved in polynomial time under the condition that
we have access to efficient probabilistic inference methods. For
example, we show that in the case of tuple-independent MLD/update
PUDs---this includes PUDs with intention models that enforce simple
conditional functional dependencies over the attribute assignments of
individual tuples---learning is solvable in polynomial time by
highly-efficient optimization methods such as stochastic gradient
descent (SGD). In fact, we show that SGD is guaranteed to recover the
true parameters of a tuple-independent PUD within error $\epsilon$ if
given access to $O(\epsilon^{-2})$ labeled examples.  }

More importantly, we establish novel results on when the intention of
a PUD can be learned from a \e{single dirty database} without access
to any labeled clean examples. Specifically, we demonstrate that under
low-noise conditions (i.e., the realizer does not cause too much
corruption in the intended data), learning the intention model corresponds
to a convex optimization problem. We also present results on when this convex optimization problem can be
solved in polynomial time.

==> sections/old_learning.tex <==
To compute requires computing $\frac{\partial}{\partial c_{l}}\log Z(\mathbf{c})$. To compute this gradient a full inference step is required. This is because, computing this gradient is equivalent to computing the expected value for each feature (corresponding to each parameter $c_{l}$) according to the distribution defined by $\mathbf{c}$~\cite{Koller:2009:PGM:1795555}.

\def\propconvex{
Given a collection $(I_j,J_j)_{j=1}^n$ of intention-realization examples and a parfactor/update PUD model where the parametric intention and realization models $\I_{\Xi}$ and $\R_{\Theta}$ correspond to parametric Gibbs distributions, the negative log-likelihood is a convex function of the parameter vector $(\Xi,\Theta)$.
}

\begin{proposition}\label{prop:convex_likelihood}
\propconvex
\end{proposition}
This proposition implies that the optimization objective for supervised learning has only global optima. Next, we discuss when this optimization problem can be solved efficiently. 

\partitle{General setting}
In general, it not computationally efficient to find an assignment $\mathbf{c}$ and $\mathbf{d}$ that minimizes the optimization objective for supervised learning.

For parfactor/update PUDs we have that $\tightcirc{\R}{\I}(I,J)\eqdef \D(I)\times  \prod_{\substack{i\in\tids(I)}} \kappa[i,I[i]](J[i])$ where 
$\D(I) = \frac{1}{Z}\,\,\times\,\,
%
\K(I)\,\,\times\,\,
%
\exp\left(
-\sum_{\varphi\in\Phi}
w(\varphi)\times |V(\varphi,I)|\right)
$. We now focus on the negative log-likelihood $l(\mathbf{c},\mathbf{d}; (I_j,J_j)_{j=1}^n)$. Given the parametric intention and realization models described in Section~\ref{sec:learningsetup}, $\mathbf{c}$ corresponds to an assignment of parameters $w_{f}$ describing $\K$ and parameters $w_\varphi = w(\varphi)$ for constraints $\Phi$. Similarly, $\mathbf{d}$ corresponds to an assignment of parameters $w_{g}$ describing $\kappa$. We use $Z(\mathbf{c})$ to denote the partition function $Z$ that corresponds to $\D$ under parameters $\mathbf{c}$. We have:
\begin{align*}
l(\mathbf{c},\mathbf{d}; (I_j,J_j)_{j=1}^n) = &-\sum_{j=1}^n\log \left(\K(I_j)\,\,\times\,\,
%
\exp\left(
-\sum_{\varphi\in\Phi}
w(\varphi)\times |V(\varphi,I_j)|\right)\right) + n\log Z(\mathbf{c})\\
&+ \sum_{j=1}^n\sum_{\substack{i\in\tids(I_j)}} \log\left(\kappa[i,I[i]](J_j[i])\right)
\end{align*}. 

For negative log-likelihood, we have the following well-known results in ML literature: There is no analytical solution to the above minimization problem~\cite{Koller:2009:PGM:1795555}, hence, iterative gradient-based methods are needed. This requires computing $\frac{\partial}{\partial c_{l}}\log Z(\mathbf{c})$. To compute this gradient a full inference step is required. This is because, computing this gradient is equivalent to computing the expected value for each feature (corresponding to each parameter $c_{l}$) according to the distribution defined by $\mathbf{c}$~\cite{Koller:2009:PGM:1795555}. However, when features introduce high-arity correlations it is well-known that marginal inference is \#P-hard~\cite{Globerson:2015:HIS:3045118.3045350}. In our setup, constraints in $\Phi$ correspond to features, hence, under generic constraints, computing the aforementioned gradient is not efficient. 

In general, one can still estimate the aforementioned gradient by using approximate inference methods such as Markov chain Monte Carlo (MCMC) methods~\cite{doi:10.1080/01621459.1993.10594284,Singh:2012:MCM:2390948.2391072} or Belief propagation~\cite{Wainwright03}. While effective in practice, these methods do not come with guarantees on the quality of the obtained solution. Next, we focus on an instance of PUD learning where exact inference is efficient and we can obtain convergence guarantees for PUD learning.

\partitle{Tuple independence} We focus on parfactor/update PUDs where all constraints in $\Phi$ are defined over one free variable. This type of parfactor/update PUDs was introduced and discuss in Section~\ref{sec:learningsetup}.  Here, each example database $(I_j,J_j)$ corresponds to one tuple identifier as tuples are independent. Moreover, the negative log-likelihood $l(\mathbf{c},\mathbf{d}; (I_j,J_j)_{j=1}^n)$ can be expressed as a sum of convex functions such that the gradient of each function can be computed efficiently. We have the following theorem:

\def\thmconvexindep{ Given a collection of $(I_j,J_j)_{j=1}^n$ intention-realization examples and a parfactor/update PUD model where the parametric intention and realization models $\I_{\Xi}$ and $\R_{\Theta}$ correspond to parametric Gibbs distributions, and each constraint $\varphi \in \Phi$ is defined over a single free variable, negative log-likelihood $l(\Xi = \mathbf{c},\Theta = \mathbf{d}; (I_j,J_j)_{j=1}^n)$ can be written as $l(\mathbf{c},\mathbf{d}; (I_j,J_j)_{j=1}^n) = \sum_{j=1}^n l^\prime(\mathbf{c},\mathbf{d}; I_j,J_j),$ where  each $l^\prime(\mathbf{c},\mathbf{d}; I_j,J_j)$ is a convex function over $\Xi$ and $Theta$ and its gradient can be evaluated in linear time with respect to $\tuples(R)$ where $R$ is the relation corresponding to the tuple identifier associated with example $(I_{j},J_{j})$.}

\begin{theorem}\label{thm:convex_indep}
\thmconvexindep
\end{theorem}
In this case, efficient convex optimization techniques such as {\em stochastic gradient descent} (SGD)~\cite{Boyd:2004:CO:993483} can be used to scale to large PUD learning instances. 

Let $\mathbf{c}$ and $\mathbf{d}$ be the parameter values obtained by solving PUD learning. Moreover, let $\mathbf{c}^\star$ and $\mathbf{d}^\star$ be the optimal parameter values that define the true intention and realization. We now bound the estimation error between $\mathbf{c}$ and $\mathbf{d}$ to $\mathbf{c}^\star$ and $\mathbf{d}^\star$ as a function of the number of available examples $(I_{j},J_{j})_{j=1}^n$. We have the following theorem:
 
\def\thmconverge{ Consider a parfactor/update PUD model where the parametric intention and realization models $\I_{\Xi}$ and $\R_{\Theta}$ correspond to parametric Gibbs distributions, and each constraint $\varphi \in \Phi$ is defined over a single free variable. Given a collection of $(I_j,J_j)_{j=1}^n$ intention-realization examples, and $\mathbf{c}$ and $\mathbf{d}$ be the parameter values obtained by solving PUD learning. We have that:
\[
	\sqrt{n} \left( \mathbf{c} - \mathbf{c}^\star \right) \rightarrow \mathcal{N}\left(0,  \Sigma^2_{\mathbf{c}^\star} \right) \text{as~} n \rightarrow \infty \text{~and~}
	\sqrt{n} \left( \mathbf{d} - \mathbf{d}^\star \right) \rightarrow \mathcal{N}\left(0, \Sigma^2_{\mathbf{d}^\star} \right) \text{as~} n \rightarrow \infty
\]
where $\Sigma^2_{\mathbf{c}^\star}$ and $\Sigma^2_{\mathbf{d}^\star}$ correspond to the asymptotic variance of estimates $\mathbf{c}$ and $\mathbf{d}$.}

\begin{theorem}\label{thm:converge}
\thmconverge
\end{theorem}

Theorem~\ref{thm:converge} states that estimators $\mathbf{c}$ and $\mathbf{d}$ obtained by solving PUD learning, converge to the true unknown parameters $\mathbf{c}^\star$ and $\mathbf{d}^\star$, and they also converge fast enough, at a rate $1/\sqrt{n}$. This result means that as the number of examples $(I_j,J_j)_{j=1}^n$ increases, the quality of our estimates becomes arbitrarily good. That is, for training data $(I_j,J_j)_{j=1}^n$, setting $n = O(\epsilon^{-2})$ suffices to achieve error $\epsilon$.

The proof of the above theorem as well as the definitions for $\Sigma^2_{\mathbf{c}^\star}$ and $\Sigma^2_{\mathbf{c}^\star}$ are presented in Appendix~\ref{sec:convergence}. The proof follows the form of standard proofs for asymptotic normality~\cite{efron1978assessing}. 
\eat{\subsection{Learning in the Presence of Training Examples}\label{sec:learnclean}

We focus on the problem of PUD learning in the presence of a collection $(Z_{i})_{i=1}^n$ of training examples. We refer the reader to Section~\ref{sec:problems} for a definition of $(Z_{i})_{i=1}^n$. The key component in our learning problem is the likelihood function, which corresponds to the objective function of an optimization problem. We now discuss the form of the likelihood function for Markov parametric PUDs, its properties, and their computational implications. Instead of optimizing the likelihood directly, we maximize the negative log-likelihood: $nll(\Xi,\Theta :T) = - \log\prod_{i=1}^n \R_{\I}(I_i, J_i)$. We have with respect to the curvature of negative log-likelihood:

\def\propconvex{
Given a collection of training examples $(Z_{i})_{i=1}^n$ and a Markov parametric PUD $(\I_{\Xi}, \R_{\Theta})$ the negative log-likelihood is a convex function of the parameter vector $(\Xi,\Theta)$.
}

\begin{proposition}\label{prop:convex_likelihood}
\propconvex
\end{proposition}

This result implies that the optimization objective for PUD learning under Markov parametric PUDs has no local optima. It does not, however, imply the uniqueness of a global optimum. For any global optimum to the MLE optimization we have that  the gradient of our negative log-likelihood objective is zero. We can compute the gradient of the negative log-likelihood as~\cite{Koller:2009:PGM:1795555} $\pd{}{\theta_{i}}\frac{1}{n}nll(\Xi, \Theta:\mathcal{D}) = \boldsymbol{E}_{\theta}[f_i] - \boldsymbol{E}_{\mathcal{D}}[f_i]$
where $f_i$ corresponds to the $i$-th element of the overall feature vector $f = (u_{\I}, u_{\R})$, parameter vector $\theta = (\Xi, \Theta)$, and $u_{\I}$ and $u_{\R}$ are the sufficient statistics describing parametric PUD $(\I_{\Xi}, \R_{\Theta})$. For the maximum likelihood estimate, we have that $\boldsymbol{E}_{\mathcal{D}}[f_i] = \boldsymbol{E}_{\thetah}[f_i]$. That is, for parameters $\thetah$ the value for each feature $f_i$ (e.g., the violations of a constraints $\phi$) relative to $P_{\theta}$ matches its empirical expectation in $D$. Unfortunately, there is no analytical form for $\theta$. It is typical to resort to iterative, gradient-based methods to improve the objective~\cite{minka}. However, to compute the gradient, a full inference step is required at every iteration of the gradient descent procedure~\cite{Koller:2009:PGM:1795555}. For general Markov PUDs the computational cost of inference can be prohibitively expensive since inference can be $\#$P-hard. Approximate inference methods such as MCMC methods~\cite{doi:10.1080/01621459.1993.10594284,Singh:2012:MCM:2390948.2391072} or Belief propagation~\cite{Wainwright03} can be used to estimate the gradient in the aforementioned optimization.

We focus on cases where inference is tractable and thus can solve PUD
learning with guarantees. Specifically, we focus on Markov parametric
PUDs that correspond to {\em MLD/update PUDs with independent tuples},
i.e., the MLD of the PUD corresponds to a tuple-independent MLD. This
means that each DC $\varphi \in \Phi$ is defined over a single free
variable. Examples of such denial constraints correspond to restricted
cases of conditional functional
dependencies~\cite{DBLP:conf/icde/BohannonFGJK07,
  Fan:2008:CFD:1366102.1366103} over the attribute values of a single
tuple, such as ``age smaller than 10 cannot co-occur with a salary
greater than \$100k'' and ``zip codes staring with 53 imply that the
state is Wisconsin.''  We have the next theorem for tuple-independent
MLD/update PUDs:

\def\thmconvexindep{
Let $\scs$ be a schema and $\U = (\I_{\Xi}, \R_{\Theta})$ be a
parametric tuple-independent MLD/update PUD. Given labeled examples
$(Z_{i})_{i=1}^n$, the negative
log-likelihood can be written as $ nll(\Xi, \Theta: D) = \sum_{k=1}^n\sum_{i \in \tids(I_k)} l(Z_i; \Xi, \Theta),$
where  $l$ is a convex function of  $\Xi$ and $\Theta$.
}

\begin{theorem}\label{thm:convex_indep}
\thmconvexindep
\end{theorem}

%\begin{theorem}
%\label{thmConvexLikelihoodIndep}
%Let $\scs$ be a schema and $\U = (\I_{\Xi}, \R_{\Theta})$ be a
%parametric tuple-independent MLD/update PUD. Given a collection
%$T=(I_1,J_1),\dots,(I_n,J_n)$ of labeled examples, the negative
%log-likelihood can be written as 
%\[
%nll(\Xi, \Theta: D) = \sum_{k=1}^n\sum_{i \in \tids(I_k)} l(I_k[i],
%J_k[i]; \Xi, \Theta),
%\]
%where  $l$ is a convex function of  $\Xi$ and $\Theta$.
%\end{theorem}

As a corollary of Theorem~\ref{thm:convex_indep}, PUD learning in this class can be solved in polynomial time, since we can use sum-of-components convex optimization techniques such as {\em stochastic gradient descent} (SGD)~\cite{Boyd:2004:CO:993483}. This is a standard results in convex optimization.

\eat{\begin{corollary}
  Let $\scs$ be a schema. $(\scs,\pudl)$-learning is solvable in
  polynomial time for the class $\pudl$ of parametric
  tuple-independent MLD/update PUDs. 
\end{corollary}}

The next step is
to bound the error of the parameter estimates $\theta = (\Xi,
\Theta)$ with respect to the optimal parameters $\theta^\star = (\Xi^\star, \Theta^\star)$ of the data
generating PUD. We show that for parametric tuple-independent MLD/update PUDs the estimated 
error is bounded as a function of the size of the example databases. 

\def\thmconverge{
Let $\scs$ be a schema and $\U = (\I_{\Xi^\star}, \R_{\Theta^\star})$ be a
parametric tuple-independent MLD/update PUD. For training collections
$T$ sampled from $\U$, estimators $(\Xi, \Theta)$ are asymptotically normal:
\begin{align*}
	\sqrt{|T|} \left( \Xi - \Xi^\star \right) &\rightarrow \mathcal{N}\left(0,  \Sigma^2_{\Xi^\star} \right) \text{as~} |T| \rightarrow \infty \text{~and~}
	\sqrt{|T|} \left( \Theta - \Theta^\star \right) &\rightarrow \mathcal{N}\left(0, \Sigma^2_{\Theta^\star} \right) \text{as~} |T| \rightarrow \infty
\end{align*}
where $\Sigma^2_{\Xi^\star}$ and $\Sigma^2_{\Theta^\star}$ correspond to the asymptotic variance of estimates $\Xi$ and $\Theta$.
}

\begin{theorem}\label{thm:converge}
\thmconverge
\end{theorem}

%\begin{theorem}
%\label{thmConvergenceIndep}
%Let $\scs$ be a schema and $\U = (\I_{\Xi^\star}, \R_{\Theta^\star})$ be a
%parametric tuple-independent MLD/update PUD. For training collections
%$T$ sampled from $\U$, estimators $(\Xi, \Theta)$ are asymptotically normal:
%\begin{align*}
%	\sqrt{|T|} \left( \Xi - \Xi^\star \right) &\rightarrow \mathcal{N}\left(0,  \Sigma^2_{\Xi^\star} \right) \text{as~} |T| \rightarrow \infty\\
%	\sqrt{|T|} \left( \Theta - \Theta^\star \right) &\rightarrow \mathcal{N}\left(0, \Sigma^2_{\Theta^\star} \right) \text{as~} |T| \rightarrow \infty
%\end{align*}
%
%
%where $\Sigma^2_{\Xi^\star}$ and $\Sigma^2_{\Theta^\star}$ correspond to the asymptotic variance of estimates $\Xi$ and $\Theta$.
%\end{theorem}

The proof of this theorem as well as the definitions for $\Sigma^2_{\Xi^\star}$ and $\Sigma^2_{\Theta^\star}$ are presented in Appendix~\ref{sec:convergence}. The proof follows the form of standard proofs for asymptotic normality~\cite{efron1978assessing}. Intuitively, Theorem~\ref{thm:converge} states that the MLE estimators not only converge to the true unknown parameters, but they converge fast enough, at a rate $1/\sqrt{|T|}$. This result means that as the size of the database increases, the quality of our estimates becomes arbitrarily good. That is, for training data $(Z_i)_{i=1}^n$, setting $n = O(\epsilon^{-2})$ suffices to achieve error $\epsilon$.
}


Consider the case when probability $p$ is fixed and independent of the number of tuple identifiers in $\D$. Moreover, 

We can optimize for the single coin allocation parameter of the realization model via simple grid-search while solving a series of convex optimization problems for $nll(\Xi,\Theta:J)$ for different fixed instantiations of $\Theta$. Recently, SGD has been shown to converge for similar simple non-convex problems~\cite{conf/icml/SaRO15,ma2017implicit}. For the above to hold $p$ should be bounded. We now show that $p$ is always bounded in the case of tuple-independent MLD/update PUDs but in the case of MLD/update PUDs with arbitrary denial constraints this is not always the case. 

If the parametric realization model $\R_{\Theta}$ is simple (i.e., we can efficiently perform grid search over the space of parameter values $\mathbf{d}$), we can minimize the overall negative log-likelihood by solving a series of convex optimization problems over $\Xi$.

%%% OLD THIGNS %%%
The results below provide preliminary insights into the
conditions under which unsupervised PUD learning can be solved
efficiently with guarantees on the estimation error for $\Xi$ and
$\Theta$.

Here, negative log-likelihood is $
nll(\Xi,\Theta: J^\star) = -\log\left(\sum_{I\in \Omega}\I_{\Xi}(I)\cdot\R_{\Theta}(J^\star|I)\right),$
where $\I_{\Xi}$ and $\R_{\Theta}$ follow the form for Markov parametric PUDs introduced in Section~\ref{sec:markovpuds}.
Similar to Section~\ref{sec:learnclean}, we focus on MLD/update PUDs and study when the negative log-likelihood is convex. For all unsupervised learning results we require that the realization model $\R$ does not introduce too much noise. More formally, we require the following condition to hold.

\partitle{Low-Noise Condition} For a class of MLD/update PUDs $\U = (\I_{\Xi},
  \R_{\Theta}, J^\star)$, we say that $\U$ satisfies the low-noise condition with respect to a probability $p$ if it is the case that for every possible $(I,J)$ in the class and every tuple identifier $i \in \varrho$ the realizer introduces an error into tuple $I[i]$ with probability at most $p$. That is, $\Pr(J[i] = I[i]| I) \ge 1 - p$.

This condition dictates a bound on the per-attribute coin
allocation of the realizer of MLD/update PUDs as a function of probability
$p$. As a result low values of $p$ enforce that the realizer does not
introduce too much corruption in the intention database. We now show that
for MLD/update PUDs and under the low-noise condition the negative log-likelihood is
a convex function of the parameters $\Xi$. We have the next theorem.

\def\convexnll{
Given a schema $\scs$ and a Markov parametric MLD/update PUD $\U = (\I_{\Xi}, \R_{\Theta}, J^\star)$ where $\Xi$ belongs in a compact convex set, there exists some fixed $p > 0$ such that whenever the low-noise condition holds w.r.t. $p$, $nll(\Xi,\Theta:J^\star)$ is a convex function of $\Xi$.
}

\begin{theorem}\label{thm:convexnll}
\convexnll
\end{theorem}

While this theorem states that under low noise the negative log-likelihood is a convex function of $\Xi$, the overall negative log-likelihood is non-convex. Convexity only provides us with guarantees on the existence of a global optimum but does not give us guarantees on the complexity of learning. Next, we study the complexity of unsupervised PUD learning.

In general, we can optimize the negative log-likelihood using non-convex optimization methods~\cite{bertsekas1999nonlinear}. If we assume simple noise model, e.g., a realization model with the same coin allocation per attribute, and assume that $p$ is bounded, we can solve PUD learning via methods such as SGD or quasi-Newton methods. We can optimize for the single coin allocation parameter of the realization model via simple grid-search while solving a series of convex optimization problems for $nll(\Xi,\Theta:J)$ for different fixed instantiations of $\Theta$. Recently, SGD has been shown to converge for similar simple non-convex problems~\cite{conf/icml/SaRO15,ma2017implicit}. For the above to hold $p$ should be bounded. We now show that $p$ is always bounded in the case of tuple-independent MLD/update PUDs but in the case of MLD/update PUDs with arbitrary denial constraints this is not always the case. 

From the proof of Theorem~\ref{thm:convexnll}, we have that for intention $\I$ with sufficient statistics $u_{\I}$ and the low noise condition probability $p$ it holds that $p \cdot \max_{J \in \Omega} \|u_\I(J)\|^2 \prec \delta \cdot I,$ where $A \prec B$ denotes that matrix $B - A$ is positive definite, $\delta >0 $ is a constant and $u_{\I}(J)$ is the sufficient statistics of $\I$ computed over $J$. For details see Appendix~\ref{sec:proofs_learning}. For this condition to hold probability $p$ may have to take a small value that depends on {\em the size of the tuple identifier repository $\varrho$} which might not be known. For example, in the presence of denial constraints, sufficient statistics $u_\I$ entail the number of violations for denial constraints, which in the worst case is proportional to the size of repository $\varrho$.

For tuple-independent PUDs $p$ is independent of the size of repository $\varrho$. Moreover, due to tuple-independence the negative log-likelihood decomposes to a sum over a series of convex functions, thus, we can solve PUD learning in polynomial time using standard sum-of-components convex optimization techniques such as SGD. We have that:

\def\convexnllindep{
Given a schema $\scs$ and a parametric tuple-independent PUD $\U = (\I_{\Xi},\R_{\Theta}, J^\star)$, parameter $p$ for Theorem \ref{thm:convexnll} to hold is independent of the number of tuple identifiers in repository $\varrho$ and the negative log-likelihood can be written as
$
  nll(\Xi,\Theta: J^\star)
  =
  \sum_{i \in \tids(J\str)} l_i(J^\star[i]; \Xi, \Theta),
$
where each $l_i$ is a convex function of $\Xi$ (keeping $\Theta$ fixed).
}

\begin{theorem}\label{cor:convexnllindep}
\convexnllindep
\end{theorem}
We focus again on MLD/update PUDs with denial constraints. From the expression on $p$ and $\|u_\I(J)\|^2$ presented above, we have: 
If we assume that the number of denial constraint violations is bounded for any $J$ sampled by a given PUD $\U$ then
$p$ will still be independent of the size of repository $\varrho$. Thus, we can use non-convex optimization methods as those for tuple-independent MLD/update PUDs to solve PUD learning.  We find this to be common in practice. Thus, an exciting future direction is to study the case of bounded violations of DCs further. 
Finally, the negative log-likelihood does not decompose to a sum
over independent random variables, thus, computing the gradient (which
requires performing inference) can be hard in the worst
case. Nonetheless, approximate inference methods as the ones discussed
in Section~\ref{sec:learnclean} can be used.


\eat{
for certain parametric intention and realization models it is possible to find a global optimum of the overall negative log-likelihood. This is when the low-noise condition holds and when $p$ is fixed and bounded. Specifically, if the parametric realization model $\R_{\Theta}$ is simple (i.e., we can efficiently perform grid search over the space of parameter values $\mathbf{d}$), we can find the global optimum for the overall negative log-likelihood by solving a series of convex optimization problems over $\Xi$ for different fixed $\Theta = \mathbf{d}$. Similar to supervised learning one can show that the negative log-likelihood decomposes as a sum over convex losses (for fixed $\Theta$) over i.i.d. examples. Moreover, the gradient of each of these losses can be computed efficiently. Hence, methods such as stochastic gradient descent can be applied to solve the corresponding optimization problem. This approach has been shown to converge for similar simple non-convex problems~\cite{conf/icml/SaRO15,ma2017implicit}.

As we mentioned, for the above to hold $p$ should be bounded. As a corollary of Theorem~\ref{thm:convexnll} we have that $p$ is always bounded in the case of Gibbs parfactor/update PUD models with unary constraints where tuples are independent. Moreover, recall that the features that characterize the intention model correspond the feature functions $F$ and the violations of constraints $\Phi$. Finally, we have that under unary constraints distribution $\D$ factorizes over individual tuple identifiers. Given the above, we have the following corollary:

\def\bounded{
Given a Gibbs parfactor/update PUD model with unary constraints  
for which the low noise condition holds, then we have for probability $p$ that $p\cdot \|C\|^2 < \delta$
where $C = \max_{R \in \scs, t \in \tuples(R), f \in F, \varphi \in \Phi}(f(t),V(\phi,t))$ and $\delta$ is a constant with $\delta > 0$.
}

\begin{corollary}\label{thm:convexnll}
\bounded
\end{corollary}
It is left as future work to investigate under which conditions $p$ is bounded for PUD models with non-unary constraints and what is the complexity and convergence properties of unsupervised PUD learning.}


==> sections/symb-table.tex <==
\section{Symbol Table}
Table~\ref{table:symb} lists the main symbols in the framework, along with their meaning.
\begin{table}
\caption{\label{table:symb}Main symbols}
\begin{tabular}{c|l}\hline
  $\scs$ & A schema. \\
  $\U$ & A PUD $(\I,\R,J\str)$.\\
  $\I$ & An intention model (probabilistic database).\\
  $\R$ & A realization model, maps every $I$ into a probabilistic database $\R_I$. \\
  $J\str$ & An observed unclean database.\\
  $\R\circs\I$ & Distribution  over pairs $(I,J)$ given by $\tightcirc{\R}{\I}(I,J)\eqdef\I(I)\cdot\R_{I}(J)$.\\
  $\U\str$ &  A probabilistic database given by $\U\str(I')=\prob_{(I,J)\sim\R\circ\I}(I=I'\mid J=J\str)$.\\
$(\D,\tau,J\str)$ & A parfactor/subset PUD.\\
$(\D,\kappa,J\str)$ & A parfactor/update PUD.\\
  $\D$ & A parfactor database $(\K,\Phi,w)$ with $w:\Phi\ra(0,\infty)$.\\
  $\K$ & A generalized tuple-independent database (generalized TID).\\
  $\Phi$ & A set of integrity constraints $\varphi$.\\
  $\tau$ & Maps $i\in\tids(R^{\D})$ to a discrete distribution $\tau[i]$ over $\tuples(R)\cup\set{\bot}$.\\
  $\kappa$ & Maps $i\in\tids(R^{\D})$ and $t\in\tuples(R)$ to a discrete distribution $\kappa[i,t]$ over $\tuples(R)$.\\
%
\hline
\end{tabular}
\end{table}

==> sections/trash.tex <==
{
A \e{tuple-independent database} (over $\scs$), or is a pair $(D,p)$
where $D$ is a database over $\scs$ and $p$ is a function that maps
every tuple identifier $i$ to a probability $p(i)\in[0,1]$. The
probability space represented by $(D,p)$ is $(\Omega,\pi)$, where
$\Omega$ consists of all the databases $E$ that are contained in $D$,
and the probability $\pi(E)$ of each $E$ is given by
\[\pi(E)\eqdef\prod_{R\in\scs}\,\,\prod_{i\in\tids_R(E)}\hskip-1em
p(i)\prod_{i\in\tids_R(D)\setminus\tids_R(E)}\hskip-2.2em(1-p(i))\,.\]
}



{
A \e{Markov Logic Network} is a tuple $(V,\Phi,w)$ where $V$ is a
finite \e{domain} of attribute values, $\Phi$ is a finite set of
logical formulas over $\scs$, possibly with free variables, and $w$
that is a function that maps every formula $\varphi\in\Phi$ to a
weight $w(\varphi)$, which can be any real number. The probability
space represented by $(V,\Phi,w)$ is $(\Omega,\pi)$, which is defined
as follows. A database $E$ in $\Omega$ is a database over $\scs$,
where each tuple $t$ of each relation $R$ consists of values from
$V$. The expression $R(t)$ is referred to as a \e{ground} fact (over
$V$). We assume a global identifier function $i_{R(t)}$ that
associates with each ground fact a unique identifier. A \e{grounding}
of formula $\varphi\in\Phi$ is obtained from $\phi$ by replacing each
free variable with a value from $V$. We denote by $\grds(V,\varphi)$
the set of all groundings of $\varphi$. For a database $E\in\Omega$
and a grounding $g\in\grds(V,\varphi)$ it is the case that $E$ either
\e{satisfies} $g$, denoted $E\models g$, or \e{violates} $g$, denoted
$E\not\models g$.  The probability $\pi(E)$ of $E$ is then given by
\[\pi(E)=\frac{1}{Z}\prod_{\varphi\in\Phi}\,\,
\prod_{\substack{g\in\grds(V,\varphi)\\ E\models g}} \hskip-1em
\exp(w(\varphi))\,.\] Here, $Z$ is a \e{normalization factor} (also
called the \e{partition function}) that normalizes the sum of
probabilities to one; that is:
\[Z\eqdef \sum_{E\in\Omega}\prod_{\varphi\in\Phi}\,\,
\prod_{\substack{g\in\grds(V,\varphi)\\ E\models g}} \hskip-1em
\exp(w(\varphi))\,.\]
}



{
A \e{tuple Markov Logic Network}, or \e{tuple-MLN} for short, is a
tuple $(D,\Phi,w)$ where $D$ is an ordinary database over $\scs$,
$\Phi$ is a finite set of logical formulas over $\scs$ (possibly with
free variables), and $w$ that is a function that maps every formula
$\varphi\in\Phi$ to a weight $w(\varphi)$, which can be any real
number. The probability space represented by $(D,\Phi,w)$ is
$(\Omega,\pi)$, where $\Omega$ consists of all the databases $E$ that
are contained in $D$, and $\pi$ is defined as follows.  A
\e{grounding} of formula $\varphi\in\Phi$ is obtained from $\phi$ by
replacing each free variable with an attribute value from $D$. We
denote by $\grds(D,\varphi)$ the set of all groundings of
$\varphi$. For a database $E\in\Omega$ and a grounding
$g\in\grds(D,\varphi)$ it is the case that $E$ either \e{satisfies}
$g$, denoted $E\models g$, or \e{violates} $g$, denoted $E\not\models
g$.  The probability $\pi(E)$ of $E$ is then given by
\[\pi(E)=
\frac{1}{Z}\times\prod_{\varphi\in\Phi}\,\,
\prod_{\substack{g\in\grds(D,\varphi)\\ E\models g}} \hskip-1em
\exp(w(\varphi))\,.\] Here, $Z$ is a \e{normalization factor} (also
called the \e{partition function}) that normalizes the sum of
probabilities to one; that is:
\[Z\eqdef \sum_{E\in\Omega}\prod_{\varphi\in\Phi}\,\,
\prod_{\substack{g\in\grds(D,\varphi)\\ E\models g}} \hskip-1em
\exp(w(\varphi))\,.\]
}




The intention model of a PUD corresponds to a probabilistic database
that defines a prior over clean databases. A \e{probabilistic
  database} over a schema $\scs$ is a probability space of (ordinary)
databases over $\scs$. All probability spaces we consider in this
paper are discrete. We next review concepts required to model the
generation of tuples in a probabilistic database and then introduce
the probabilistic database representations considered in this paper.

\partitle{Tuple Generation} We review basic concepts related to tuple
generation that are necessary to define the probabilistic database
representations introduced below. Let $\scs$ be a schema. An
\e{identifier repository} for $\scs$ consists of pairwise-disjoint
collections of tuple identifiers for each relation symbol. Formally,
an identifier repository is a function $\varrho$ that maps every
relation symbol $R$ into a finite set, denoted $\varrho_R$, of tuple
identifiers, such that $\varrho_R\cap \varrho_S=\emptyset$ whenever
$R\neq S$. A \e{per-table coin allocation} for $\scs$ is a function
$p$ that maps every relation symbol $R$ into a probability (i.e., a
number in $[0,1]$), denoted $p_R$. A \e{per-column coin allocation}
(\e{for $\scs$}) is a function $p$ that maps every relation symbol $R$
and attribute $A$ of $R$ into a probability, denoted $p_{R.A}$. We now
define mechanisms for generating random attribute values and random
tuples. We define a \e{value generator} for $\scs$ to be a function
$\vg$ that maps every relation $R$ and attribute $A$ of $R$ into a
distribution, denoted $\vgra$, over atomic values. We also define a
\e{tuple generator} for $\scs$ to be a function $\tg$ that maps every
relation symbol $R$ into a distribution, denoted $\tgr$, over tuples
of $R$. We can define a tuple generator $\tg$ via a value generator
$\vg$---a tuple in $R$ is generated by independently sampling a value
from $\vgra$ for each attribute $A$. In general, a tuple generator may
introduce correlations across attributes. We assume that given a tuple
$t$ and an atomic value $a$, probabilities $\tgr(t)$ and $\vgra(a)$
can be computed in polynomial time.




  \partitle{Probabilistic Database Representations} We consider two
  representations: (1) \e{Tuple Independent and Identically
    Distributed} (TIID) databases that correspond to a simplified form
  of tuple independent databases, and (2) \e{Markov Logic Databases}
  (MLDs) that extend TIIDs with constraints over tuples following the
  semantics of \e{Markov
    Logic}~\cite{Richardson:2006:MLN:1113907.1113910}.

Let $\scs$ be a schema.  A database \e{with independent, identically distributed tuples}, or \e{TIID} for short, is a triple $(\varrho,p,\tg)$ such that $\varrho$ is an identifier repository, $p$ is a per-table coin allocation, and $\tg$ is a tuple generator. Semantically, a TIID $\P=(\varrho,p,\tg)$ defines a probabilistic database via the following generative process: For each identifier $i$ in $\varrho$, randomly choose, with probability $p$, whether or not to generate a tuple for $i$; if so, then generate the tuple using $\tg$. More formally, the possible worlds are the databases $D$ with $\tids_R(D)\subseteq \varrho_R$ for all relation symbols $R$, and the probability $\P(D)$ of $D$ is defined as $\P(D)\eqdef\prod_{R\in\scs}\P(R^D)$ where each $\P(R^D)$ is given by
$\P(R^D)\eqdef\prod_{\substack{i\in\tids_R(D)}}\left(p_R\cdot\tgr(D[i])\right)
\times\prod_{\substack{i\in \varrho_R\setminus
    \\\tids_R(D)}}\hspace{-0.5em}(1-p_R)\,.$

A \e{Markov Logic Database} (\e{MLD}) is a triple $(\P,\Phi,w)$ where: (1) $\P$ is a TIID, (2) $\Phi$ is a finite set of DCs, and (3) $w$ is a \e{penalty function} that associates every formula
  $\varphi\in\Phi$ with a positive weight $w(\varphi)$. Semantically, an MLD $\M=(\P,\Phi,w)$ defines a probabilistic database as follows: The possible worlds are those of $\P$. The probability $\M(D)$ of a possible world $D$ is given by $\M(D)\eqdef\frac{1}{Z}\times\P(D)\times\prod_{\varphi\in\Phi}e^{-w(\varphi)\cdot |V(D,\varphi)|}$ where $V(D,\varphi)$ is the set of all violations of $\varphi$ in $D$, and $Z$ is a \e{normalization factor} (a.k.a. \e{partition function}) that normalizes the total sum of probabilities to one. We use $w(\varphi)=\infty$ for \e{hard} constraints.

\eat{
 which allows for uncertainty on the values in tuples
as well as the existence of the tuples. An MLD extends a {\em Tuple
  Independent Database} (TID) with correlations across attribute
assignments over tuples and correlations across tuples captured via
Markov Logic Networks (MLNs). The generative model for an MDD starts
with a database with {\em empty cells}. For each tuple it determines
independently whether the tuple exists, {\em and if so}, what its
attributes are.
}

\eat{
\subsubsection{Tuple Independent Relation (TIR)} To define a TID, we
first define a {\em Tuple Independent Relation} (TIR) $R$. Let $R$ be
a relation symbol of $\scs$. Let $T_R$ be a set of tuple identifiers
and let $R$ be a $k-ary$ relation with attribute $\sig(R)$. Let
$dom(R) = dom(A_1) \times dom(A_2 )\dots \times dom(A_k)$ be the set
of possible assignments to a tuple in $R$; here $dom(A_i)$ denotes the
set of possible assignments to the $i$-th attribute of a tuple. The
set of possible worlds, that is the set of possibles instances we
could observe for TIR $R$ is $\Omega_R: T_R \pfun dom(R)$, the set of
partial functions from tuple identifiers in $R$ to tuple values. The
probability of such as partial function is fully characterized by two
components:
\begin{itemize}
	\item A {\em tuple-selection probability} $p_R \in [0,1]$
	\item A generator function $\delta_R: dom(A_1) \times dom(A_2
          )\dots \times dom(A_k) \rightarrow [0,1]$ that maps
          attribute assignments to a probability distribution. Let
          $r[i]$ be the attribute assignment generated for a tuple
          with identifier $i$ in a relation $r$ for symbol $R$. We
          denote $\delta_R(r[i])$ the probability associated with that
          attribute-value assignment.
\end{itemize}
Eventually a TIR over a relation symbol $R$ of $\scs$ is a tuple
$(T_R,p_R,\delta_R)$ where the probability of a relation $r$ sampled
by $R$ is given by: {\scriptsize \[\pi(r)\,\,\eqdef\,\,
%
\left(
%
\prod_{i\in\tids(r)}p\cdot
%
\delta_R(r[i])
%
\right)
%
\cdot
%
\left(
%
\prod_{i\in T_R\setminus\tids(r)}(1-p_R)
%
\right)
%
%
\]}
Or, in a simplified form:
{\scriptsize
\[\pi(r)\,\,\eqdef\,\,
%
p_R^{|r|}\cdot(1-p_R)^{|T_R|-|r|}\cdot
%
\prod_{i\in\tids(r)}\delta_R(r[i])
%
%
\]}
where $\tids(r)$ is the set of tuple identifiers present in $r$.

\noindent\textbf{MLN-TIR} An MLN tuple independent relation $R$ is 
defined as a tuple $(T_R,p_R,\delta_R)$ where the value generator
$\delta_R$ is described by an MLN. Specifically, let $\Phi_R$ be a set
of logical formulas with free variable that can range over $T_R$, and
which express propositions about a single database. That is, its
atomic terms are of the form $r_j(i)$ where $i$ is a free variable
that ranges over $T_R$, $j$ is the index of an attribute, and $a \in
dom(A_j)$ is a value that attribute $A_j$ can take on. We further
require that every logical formula $\phi \in \Phi_R$ has at most one
free variable. Let $w_R: \Phi_R \rightarrow \mathbb{R}$ be a function
that assigns a {\em weight} to each formula in $\Phi_R$. This weight
can be a fixed real number or it can be a vector of model parameters
$\theta_R$; more precisely $w_R$ is an affine function of
$\theta_R$. Then the probability of a relation $r$ sampled from $R$
has probability: {\scriptsize
\[\pi(r)\,\,=\,\,
%
p_R^{|r|}\cdot(1-p_R)^{|T_R|-|r|}\cdot
%
\frac{1}{Z}\exp\sum_{i \in \tids(r)}\sum_{\varphi\in\Phi_R}\,\,
\sum_{\substack{g\in\grds(V,\varphi)\\ r\models g}} w_{R}(\phi) 
%
%
\]}
where $Z$ is a \e{normalization factor} (also called the \e{partition
  function}) that normalizes the sum of probabilities to one.

\subsubsection{Tuple Independent Database (TID)} A {\em Tuple
  Independent Database} (TID) $\K$ (over $\scs$) maps every relation
symbol $R$ of $\scs$ to a TIR, denoted $R^\K$, over $R$. Semantically,
the generative process of $\K$ produces a relation of each $R$
independently from the others. In other words, the generative models
defined by $R$ constructs a random database $I$ as follows:
\begin{algorithm}
\begin{algorithmic}
\FORALL{$R\in\scs$}
\STATE independently generate a random relation $r$ from $R^{\K}$
\STATE assign $R^I=r$
\ENDFOR
\end{algorithmic}
\end{algorithm}
For a TID $\K$, we denote by $\Omega(\K)$ the sample space of the
probability space defined by $\K$, and for $I\in\Omega(\K)$ we denote
by $\prob_{\K}(I)$ the probability of $I$ under that probability
space. Finally, we denote by $\tids_R(\K)$ the set of all tuple
identifiers that appear in the TIR $R^{\K}$.

Similar to MLN-TIR an {\em MLN-TID} is a TID where the value generator $\delta_R$ for each relation symbol $R \in \scs$ is defined by an MLN.

\subsubsection{Markov Logic Database}\label{sec:mldb}
We extend a TID with the ability to introduce bias towards
\e{dependencies} across tuples (such as FDs). We do so by enhancing
the definition of a TID with a \e{Markov Logic Network} that captures
correlations across tuples. We refer to such a probabilistic database
as a {\em Markov Logic Database} (MLD). An MLD consists of a TID,
along with set of weighted formulas. Formally, an MLD (over $\scs$) is
a tuple $(\K,\Phi,\w)$ where:
\begin{itemize}
\item $\K$ is a TID;
\item $\Phi_C$ is a finite collection of formulas with free variables
  in \e{tuple-relational calculus} over $\scs$;
\item $w_C: \Phi_C \rightarrow \mathbb{R}$ be a function that assigns a weight to each formula in $\Phi_C$.
\end{itemize}
An example of a formula in $\Phi$ is the violation of an FD
$R:A\rightarrow B$.
\[x\in R\land y\in R\land x.A=y.A\land x.B\neq y.B\] We assume that
every formula in $\Phi_C$ is \e{safe} (and in particular domain
independent)---in fact, this safety is automatic from the fact that we
consider the free variables (here $x$ and $y$) to range over tuples in
$\K$. Moreover, if $\varphi\in\Phi_C$ has the free variables
$x_1,\dots,x_k$, then we assume that $\phi(x_1,\dots,x_k)$ is of the
form:
\[x_1\in R_1\land\dots\land x_k\in R_k\land\psi(x_1,\dots,x_k)\,.\]

The probability space $(\Omega,\pi)$ defined by $(\K,\Phi_C,w_C)$ has
the same sample space as $\K$, but the probability $\pi(I)$ of each
random database is defined as follows: Let $\varphi$ be a formula in
$\Phi_C$ and $I$ a database over $\scs$.  A \e{true realization} of
$\varphi$ in $I$ is an assignment of tuples from $I$ to the free
variables of $\varphi$ that make $\varphi$ true in $I$.  We denote by
$\tau(\varphi,I)$ the set of all true realizations of $\varphi$ in
$I$. The probability of $I$ is defined:
\[
\pi(I)\eqdef
%
\prob_{\K}(I)
%
\cdot
%
\frac{1}{Z}
%
\exp\sum_{\varphi\in\Phi_C}\sum_{\varrho\in\tau(\varphi,I)}
%
w_C(\varphi)
\]

Here, $Z$ is a \e{normalization factor} (also called the \e{partition
  function}) that normalizes the sum of probabilities to one:
\[Z\eqdef 
%
\sum_{J\in\Omega(\I)}
%
\,\,
%
\prod_{\varrho\in\tau(\varphi,J)}
%
\exp(w_C(\varphi))
\]

If TID $\K$ corresponds to an MLN-TID then the overall probability of
an MLD $(\K, \Phi_C, w_C)$ can be expressed as a single {\em
  exponential family model}. The exponential family of distributions
provides a general framework for specifying a parameterization of a
distribution in terms of natural parameters called the {\em natural
  sufficient statistics} of the family. For an MLD $(\K, \Phi_C, w_C)$
we have that the corresponding parameterized exponential family is:
\begin{align*}	
\pi(I) &= 
%
\frac{1}{Z}\exp\sum_{R \in \scs}\sum_{i \in T_R} \left(\log(\frac{p_R}{1 - p_R})E[i]+ \log(1-p_R)\right) \\
%
&\cdot \exp\sum_{R \in \scs}\sum_{i \in \tids(r)}\sum_{\varphi\in\Phi_R}\,\,
\sum_{\substack{g\in\grds(V,\varphi)\\ r\models g}} w_{R}(\phi) \\
%
&\cdot \exp\sum_{\varphi\in\Phi_C}\sum_{\varrho\in\tau(\varphi,I)}
%
w_C(\varphi)
\end{align*}
where $E[i]$ is an atomic predicate that takes the value \texttt{True}
if tuple with identifier $i$ exists in $I$ and \texttt{False}
otherwise.

\noindent\textbf{Parameterized MLD} Let $T = \bigcup_{R \in
  \scs}T_R$. A {\em parameterized MLD} corresponds to an MLN over
propositions $\Phi = \{\{E[i]\}_{i \in T}, \{\Phi_R\}_{R \in \scs},
\Phi_C\}$ whose atomic terms are of the form
\[
  r_j(i) = a \text{\hspace{2em}or\hspace{2em}} i \in \text{dom}(r)
\]
where $i$ is a free variable that ranges over $T = \bigcup_{R \in scs}
T_R$, $j$ is the index of an attribute, and $a \in dom(A_j)$ is a
value that attribute can take on. Then an MLD is defined over $\Omega$
as
\[
  \pi_{\btheta}(I)
  =
  \frac{1}{Z}
  \exp\left(
    \sum_{\varphi \in \Phi}
    \sum_{\substack{g \in \grds(T, \varphi) \\ I \models g}}
    w_I(\varphi)
  \right).
\]
where $w: \Phi \rightarrow \R$ is a function that assigns a
\emph{weight} to each formula in $\Phi$ with $w$ being an affine
function of $\btheta$.


}

==> sections/unsupervised.tex <==
We now present preliminary results for unsupervised
$(\scs,\pudl)$-learning. We are given a training collection
$(J_j)_{j=1}^n$ and seek to find $\mathbf{c}$ and $\mathbf{d}$ that
minimize the negative log-likelihood $l(\Xi =
\mathbf{c},\Theta=\mathbf{d}; (J_j)_{j=1}^n) =
-\sum_{j=1}^n\log\sum_{I}\tightcirc{\R}{\I}(I,J_j)$. 
Again, there is no analytical solution
for finding optimal $\mathbf{c}$ and $\mathbf{d}$. Hence, one needs to
use iterative gradient-based approaches, and again the questions of
convexity and gradient computation arise.  In the general case, this
function is \e{not} necessarily convex. Hence, gradient-based methods
are not guaranteed to converge to a global optimum. However, one can
still solve the corresponding optimization problem using non-convex
optimization methods~\cite{bertsekas1999nonlinear}. Nonetheless, we
show next that when realizers do not introduce \e{too much error}, we
can establish guarantees.

\subparagraph*{Low-noise condition} Consider a Gibbs parfactor/update PUD
model. We say that a PUD defined by $\I_{\Xi/\mathbf{c}}$ and
$\R_{\Theta/\mathbf{d}}$ satisfies the \e{low-noise condition} with
probability $p$ if the realizer introduces an
error with probability at most $p$. That is, for all intensions $I$
and identifiers $i\in\tids(I)$, it is the case that $\prob(J[i] =
I[i]|I) \ge 1 - p$. We have the following.

\def\convexnll{ Consider a Gibbs parfactor/update PUD model where
  $\Xi$ takes values from a compact convex set. Given a training
  collection $(J_j)_{j=1}^n$, there exists a fixed probability $p > 0$
  such that, under the low-noise condition with probability $p$,
  the negative log-likelihood $l(\Xi = \mathbf{c},\Theta=\mathbf{d};
  (J_j)_{j=1}^n)$ is a convex function of $\Xi$.  }

\begin{theorem}\label{thm:convexnll}
\convexnll
\end{theorem}
Hence, in certain cases, it is possible to find a global optimum of
the overall negative log-likelihood. For that, the low-noise condition
should hold with probability $p$ that is also bounded, that is, it
cannot be arbitrarily large.  We can show that, if the low-noise
condition holds with probability $p$, it is indeed bounded for Gibbs
parfactor/update PUDs with unary constraints (see the extended version of our paper~\cite{DBLP:journals/corr/abs-1801-06750}). We then find a global
optimum as follows.  We assume a simple parametric realization
$\R_{\Theta}$, that is, a model for which we can efficiently perform
\e{grid search} over the space of parameter values $\mathbf{d}$. To
find the global optimum for the negative log-likelihood, we solve a
series of convex optimization problems over $\Xi$ for different fixed
$\Theta = \mathbf{d}$. For each of these problems, we are guaranteed
to find a corresponding global optimum $\mathbf{c}$, and by performing
a grid search we are guaranteed to find the overall global optimum
$\mathbf{c}$ and $\mathbf{d}$. This approach has been shown to
converge for similar simple non-convex
problems~\cite{conf/icml/SaRO15,ma2017implicit}.

Finally, similarly to supervised learning, the negative log-likelihood
for fixed $\Theta=\mathbf{d}$ decomposes into a sum of convex losses
over $(J_j)_{i=1}^n$ where each example $J_j$ contains a single
tuple. We use $J_j[0]$ to denote that tuple. We have that $l(\Xi =
\mathbf{c}, \Theta=\mathbf{d}, (J_j)_{j=1}^n) = \sum_{j=1}^n
l^{\prime}(\mathbf{c},\mathbf{d};J_j[0])$ where $\mathbf{d}$ is
fixed. We show that the gradient of each
$l^{\prime}(\mathbf{c},\mathbf{d};J[0])$ can be evaluated in polynomial time to $\tuples(R)$ where $R$ is the relation corresponding to
the tuple identifier associated with the example $(J_j)$.

\def\thmconvexunsup{Given a training collection $(J_j)_{j=1}^n$ and a
  Gibbs parfactor/update PUD model with unary constraints that
  satisfies the low-noise condition with probability $p$, the exact
  gradient of $l(\Xi = \mathbf{c},\Theta = \mathbf{d}; (J_j)_{j=1}^n)$
  with respect to $\Xi$ can be evaluated in time $O(n\cdot \max_{R \in
    \scs}|\tuples(R)|^2)$ for every fixed $\mathbf{d}$.}

It is left for future work to find sufficient conditions for $p$ to be
bounded for PUD models with more general constraints, as well as the
complexity and convergence aspects.
%%%%% PLease do not erase this %%%
\eat{
for certain parametric intention and realization models it is possible to find a global optimum of the overall negative log-likelihood. This is when the low-noise condition holds and when $p$ is fixed and bounded. Specifically, if the parametric realization model $\R_{\Theta}$ is simple (i.e., we can efficiently perform grid search over the space of parameter values $\mathbf{d}$), we can find the global optimum for the overall negative log-likelihood by solving a series of convex optimization problems over $\Xi$ for different fixed $\Theta = \mathbf{d}$. Similar to supervised learning one can show that the negative log-likelihood decomposes as a sum over convex losses (for fixed $\Theta$) over i.i.d. examples. Moreover, the gradient of each of these losses can be computed efficiently. Hence, methods such as stochastic gradient descent can be applied to solve the corresponding optimization problem. This approach has been shown to converge for similar simple non-convex problems~\cite{conf/icml/SaRO15,ma2017implicit}.

As we mentioned, for the above to hold $p$ should be bounded. As a corollary of Theorem~\ref{thm:convexnll} we have that $p$ is always bounded in the case of Gibbs parfactor/update PUD models with unary constraints where tuples are independent. Moreover, recall that the features that characterize the intention model correspond the feature functions $F$ and the violations of constraints $\Phi$. Finally, we have that under unary constraints distribution $\D$ factorizes over individual tuple identifiers. Given the above, we have the following corollary:

\def\bounded{
Given a Gibbs parfactor/update PUD model with unary constraints  
for which the low noise condition holds, then we have for probability $p$ that $p\cdot \|C\|^2 < \delta$
where $C = \max_{R \in \scs, t \in \tuples(R), f \in F, \varphi \in \Phi}(f(t),V(\phi,t))$ and $\delta$ is a constant with $\delta > 0$.
}

\begin{corollary}\label{thm:convexnll}
\bounded
\end{corollary}
It is left as future work to investigate under which conditions $p$ is bounded for PUD models with non-unary constraints and what is the complexity and convergence properties of unsupervised PUD learning.}
